Taming the Beast: Learning to Control Neural Conversational Models

This thesis investigates the controllability of deep learning-based, end-to-end, generative dialogue systems in both task-oriented and chit-chat scenarios. In particular, we study the different aspects of controlling generative dialogue systems, including controlling styles and topics and continuously adding and combining dialogue skills. In the three decades since the first dialogue system was commercialized, the basic architecture of such systems has remained substantially unchanged, consisting of four pipelined basic components, namely, natural language understanding (NLU), dialogue state tracking (DST), a dialogue manager (DM) and natural language generation (NLG). The dialogue manager, which is the critical component of the modularized system, controls the response content and style. This module is usually programmed by rules and is designed to be highly controllable and easily extendable. With the emergence of powerful "deep learning" architectures, end-to-end generative dialogue systems have been proposed to optimize overall system performance and simplify training. However, these systems cannot be easily controlled and extended as the modularized dialogue manager can. This is because a single neural system is used, which is usually a large pre-trained language model (e.g., GPT-2), and thus it is hard to surgically change desirable attributes (e.g., style, topics, etc.). More importantly, uncontrollable dialogue systems can generate offensive and even toxic responses. Therefore, in this thesis, we study controllable methods for end-to-end generative dialogue systems in task-oriented and chit-chat scenarios. Throughout the chapters, we describe 1) how to control the style and topics of chit-chat models, 2) how to continuously control and extend task-oriented dialogue systems, and 3) how to compose and control multi-skill dialogue models.

==> 2_authorization.tex <==
\null\skip0.2in
\begin{center}
{\bf \Large \underline{Authorization}}
\end{center}
\vspace{12mm}

I hereby declare that I am the sole author of the thesis.

\vspace{10mm}

I authorize the Hong Kong University of Science and Technology to lend this
thesis to other institutions or individuals for the purpose of scholarly research.

\vspace{10mm}

I further authorize the Hong Kong University of Science and Technology to
reproduce the thesis by photocopying or by other means, in total or in part, at the
request of other institutions or individuals for the purpose of scholarly research.

\vspace{30mm}

\begin{center}
\underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~}\\
~~~~\thesisauthor \\
~~~~\signdate

\end{center}


==> 3_signature.tex <==
\begin{center}
{\Large \thesistitle}\\
\vspace{5mm}
by\\
\vspace{3mm}
\thesisauthor\\
\vspace{5mm}
This is to certify that I have examined the above PhD thesis\\
and have found that it is complete and satisfactory in all respects,\\
and that any and all revisions required by\\
the thesis examination committee have been made.
\end{center}

\vspace{12mm}

\begin{center}
\underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ }\\
\supervisorinfo
\end{center}

% \vspace{15mm}
% \begin{center}
% \underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ }\\
% \cosupervisorinfo
% \end{center}

\vspace{12mm}
\begin{center}
\underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ }\\
\depheadinfo
\end{center}

\vspace{4mm}

\textbf{Thesis Examination Committee}
\TabPositions{5cm}
\begin{enumerate}[itemsep=-4.0mm]
    \item Prof. Pascale Fung \tab Department of Electronic and Computer Engineering
    \item Prof. Bertram Shi \tab Department of Electronic and Computer Engineering
    \item Prof. Qifeng Chen \tab Department of Electronic and Computer Engineering
    \item Prof. Ma Xiaojuan  \tab Department of Computer Science and Engineering
    \item Prof. David Cheng Chang \tab Department of Humanities
    \item Prof. Yun-Nung Chen \tab Department of Computer Science and Information Engineering, National Taiwan University
\end{enumerate}


\vspace{5mm}
\begin{center}
\departmentname\\
\vspace{1mm}
\signdate
\end{center}


==> 4_dedicate.tex <==
\thispagestyle{empty}
\null\vskip0.5in
\begin{center}


  \vspace{20mm}

  \begin{LARGE}
    \dedicate
  \end{LARGE}

  \vspace{4mm}



\end{center}

\vfill


==> 5_acknowledgement.tex <==
\centerline{{\bf \Large Acknowledgments}} \vspace{5mm} \noindent

Firstly, I would like to express my most sincere gratitude to my supervisor, Professor Pascale Fung, for her knowledgeable guidance and supervision throughout my PhD. She is the one that suggested that I work on dialogue systems before it was as popular a topic as it is now. She has, indeed, a great research vision, which I have constantly been learning from, and which allowed me to constantly grow as a researcher.   

Next, I would like to express my appreciation to Professor Bertram Shi, Professor Qifeng Chen, Professor Xiaojuan Ma, and Professor David Cheng Chang for taking their time to be on my thesis examining committee. I am also thankful to Professor Yun-Nung Chen, who has inspired me with many of her seminal works on task-oriented dialogue systems, and it is my pleasure to have her on my thesis committee. I would like to also thanks Professor Francesco Ciucci, for his academic and professional advice during my four years in HKUST. I want to give my gratitude to Tania Leigh Wilmshurst, who proofread my papers and thesis countless times, and gave me insightful and useful advice on academic writing.

In the last four years, I have had an exciting journey in the lab with amazing lab friends and colleagues. Therefore, I want to thank Genta Indra Winata, Chien-Sheng Wu, Zhaojiang Lin, Nayeon Lee, and Peng Xu for the many collaborations over the years. My thanks go to Chien-Sheng Wu for the great collaborations on dialogue related projects; I always enjoyed our time having discussions and working together; to Genta Indra Winata for the multiple great collaborations on speech and code-switching related projects; to Zhaojiang Lin for the continuous and insightful discussions on dialogue systems research; to Nayeon Lee for the great work together on bias related projects; and to Peng Xu for the constructive discussions on NLP methods and research directions. Thanks also go to Onno Kampman, Ji Ho Park and Dario Bertero, who provided guidance at the beginning of my PhD, and to Zihan Liu, Jamin Shin, Yejin Bang, Samuel Cahyawijaya, Yan Xu, Etsuko Ishii, Elham Barezi, Tiezheng Yu, Ziwei Ji, and many others for the invaluable research experiences. 

I would further like to express my thanks to Sumanth Dathathri for the infinite number of research discussions and for the language model related projects. I would also like to thank the MLCollective members Rosanne Liu and Jason Yosinski for their insightful feedback on my work and for the great collaboration opportunity they gave me. Thanks to the ex UberAI researchers Mahdi Namazifar, Piero Molino, Gökhan Tür, Alexandros Papangelis, Huaixiu Zheng, Dian Yu, Chandra Khatri, Adrien Ecoffet, and Joost Huizinga for their support and great research interactions during my internship, and thanks to the FacebookAI researchers Zhiguang Wang, Seungwhan Moon, Zhenpeng Zhou, Paul Crook, Bing Liu, Zhou Yu, and Eunjoon Cho for their support and great research discussion during my internship there. 


Finally, I would like to express my gratitude to all my friends in Hong Kong, and many others who have motivated me during all the challenging times. I enjoyed every moment that we spent together, especially our Sunday lunches. I want to thank Colan Chen, my flatmate and friend, for helping with drawing the dragons in this thesis and for other drawing used in other research papers (e.g., PPLM). I want to thank my family for supporting me all the way during my PhD. Last but not least, I would like to thank my wife (Zhang YingYao a.k.a. bao bao) who has always been there in making any decision, hard or easy.  

==> publication.tex <==
\null\skip0.2in
\begin{center}
{\bf \Large \underline{List of Publications}}
\end{center}
\vspace{12mm}

\paragraph{Conference Papers (sorted by date)}

\begin{itemize}
\item Continual Learning in Task-Oriented Dialogue Systems. Andrea Madotto, Zhaojiang Lin, Zhenpeng Zhou, Seungwhan Moon, Paul Crook, Bing Liu, Zhou Yu, Eunjoon Cho, Zhiguang Wang. Under submission at EMNLP 2021.  
\item Towards Few-Shot Fact-Checking via Perplexity. Nayeon Lee, Yejin Bang, Andrea Madotto, Madian Khabsa, Pascale Fung. In Proceedings of the 2021 North American Chapter of the Association for Computational Linguistics, NAACL 2021. 
\item The Adapter-Bot: All-In-One Controllable Conversational Model. Andrea Madotto, Zhaojiang Lin, Yejin Bang, and Pascale Fung. In The Thirty-Fifty AAAI Conference on Artificial Intelligence, AAAI 2021.
\item CrossNER: Evaluating Cross-Domain Named Entity Recognition. Zihan Liu, Yan Xu, Tiezheng Yu, Wenliang Dai, Ziwei Ji, Samuel Cahyawijaya, Andrea Madotto, and Pascale Fung. In The Thirty-Fifty AAAI Conference on Artificial Intelligence, AAAI 2021. 
\item On the Importance of Word Order Information in Cross-lingual Sequence Labeling. Zihan Liu, Genta Indra Winata, Samuel Cahyawijaya, Andrea Madotto, Zhaojiang Lin, and Pascale Fung. In The Thirty-Fifty AAAI Conference on Artificial Intelligence, AAAI 2021. 
\item Learning Knowledge Bases with Parameters for Task-Oriented Dialogue Systems. Andrea Madotto, Samuel Cahyawijaya, Genta Indra Winata, Yan Xu, Zihan Liu, Zhaojiang Lin, and Pascale Fung. In Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing: Findings, EMNLP 2020, Online Event, 16-20 November 2020.
\item Plug-and-Play Conversational Models. Andrea Madotto, Etsuko Ishii, Zhaojiang Lin, Sumanth Dathathri, and Pascale Fung. In Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing: Findings, EMNLP 2020, Online Event, 16-20 November 2020.
\item Exploring Versatile Generative Language Model Via Parameter-Efficient Transfer Learning. Zhaojiang Lin, Andrea Madotto, and Pascale Fung. In Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing: Findings, EMNLP 2020, Online Event, 16-20 November 2020.
\item MinTL: Minimalist Transfer Learning for Task-Oriented Dialogue Systems. Zhaojiang Lin, Andrea Madotto, Genta Indra Winata, and Pascale Fung. In Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing, EMNLP 2020, Online, November 16-20, 2020
\item Generating Empathetic Responses by Looking Ahead the User’s Sentiment. Jamin Shin, Peng Xu, Andrea Madotto, and Pascale Fung. In 2020 IEEE International Conference on Acoustics, Speech and Signal Processing, ICASSP 2020, Barcelona, Spain, May 4-8, 2020.
\item Plug and Play Language Models: A Simple Approach to Controlled Text Generation. Sumanth Dathathri, Andrea Madotto, Janice Lan, Jane Hung, Eric Frank, Piero Molino, Jason Yosinski, and Rosanne Liu. In 8th International Conference on Learning Representations, ICLR 2020, Addis Ababa, Ethiopia, April 26-30, 2020.
\item Exploration Based Language Learning for Text-Based Games. Andrea Madotto, Mahdi Namazifar, Joost Huizinga, Piero Molino, Adrien Ecoffet, Huaixiu Zheng, Alexandros Papangelis, Dian Yu, Chandra Khatri, and Gökhan Tür. In Proceedings of the Twenty-Ninth International Joint Conference on Artificial Intelligence, IJCAI 2020.
\item Learning Fast Adaptation on Cross-Accented Speech Recognition. Genta Indra Winata, Samuel Cahyawijaya, Zihan Liu, Zhaojiang Lin, Andrea Madotto, Peng Xu, and Pascale Fung. In Interspeech 2020, 21st Annual Conference of the International Speech Communication Association, Virtual Event, Shanghai, China, 25-29 October 2020.
\item Getting To Know You: User Attribute Extraction from Dialogues. Chien-Sheng Wu, Andrea Madotto, Zhaojiang Lin, Peng Xu, and Pascale Fung. In Proceedings of The 12th Language Resources and Evaluation Conference, LREC 2020, Marseille, France, May 11-16, 2020 2020.
\item Transferable Multi-Domain State Generator for Task-Oriented Dialogue Systems. Chien-Sheng Wu, Andrea Madotto, Ehsan Hosseini-Asl, Caiming Xiong, Richard Socher, and Pascale Fung. In Proceedings of the 57th Conference of the Association for Computational Linguistics, ACL 2019, Florence, Italy, July 28- August 2, 2019, Volume 1: Long Papers 2019.
\item Personalizing Dialogue Agents via Meta-Learning. Andrea Madotto, Zhaojiang Lin, Chien-Sheng Wu, and Pascale Fung. In Proceedings of the 57th Conference of the Association for Computational Linguistics, ACL 2019, Florence, Italy, July 28- August 2, 2019, Volume 1: Long Papers 2019
\item Attention over Parameters for Dialogue Systems. Andrea Madotto, Zhaojiang Lin, Chien-Sheng Wu, Jamin Shin, and Pascale Fung. NeurIPS-ConvAI Workshop 2019.
\item Exploring Social Bias in Chatbots using Stereotype Knowledge. Nayeon Lee, Andrea Madotto, and Pascale Fung. In Proceedings of the 2019 Workshop on Widening NLP\@ACL 2019, Florence, Italy, July 28, 2019.
\item Code-Switched Language Models Using Neural Based Synthetic Data from Parallel Sentences. Genta Indra Winata, Andrea Madotto, Chien-Sheng Wu, and Pascale Fung. In Proceedings of the 23rd Conference on Computational Natural Language Learning, CoNLL 2019, Hong Kong, China, November 3-4, 2019.
\item MoEL: Mixture of Empathetic Listeners. Zhaojiang Lin, Andrea Madotto, Jamin Shin, Peng Xu, and Pascale Fung. In Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing, EMNLP-IJCNLP 2019, Hong Kong, China, November 3-7, 2019.
\item Zero-shot Cross-lingual Dialogue Systems with Transferable Latent Variables. Zihan Liu, Jamin Shin, Yan Xu, Genta Indra Winata, Peng Xu, Andrea Madotto, and Pascale Fung. In Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing, EMNLP-IJCNLP 2019, Hong Kong, China, November 3-7, 2019.
\item Clickbait? Sensational Headline Generation with Auto-tuned Reinforcement Learning. Peng Xu, Chien-Sheng Wu, Andrea Madotto, and Pascale Fung.In Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing, EMNLP-IJCNLP 2019, Hong Kong, China, November 3-7, 2019.
\item CAiRE\_HKUST at SemEval-2019 Task 3: Hierarchical Attention for Dialogue Emotion Classification. Genta Indra Winata, Andrea Madotto, Zhaojiang Lin, Jamin Shin, Yan Xu, Peng Xu, and Pascale Fung. In Proceedings of the 13th International Workshop on Semantic Evaluation, SemEval\@NAACL-HLT 2019, Minneapolis, MN, USA, June 6-7, 2019.
\item Mem2Seq: Effectively Incorporating Knowledge Bases into End-to-End Task-Oriented Dialog Systems. Andrea Madotto, Chien-Sheng Wu, and Pascale Fung. In Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics, ACL 2018, Melbourne, Australia, July 15-20, 2018, Volume 1: Long Papers 2018.
\item Code-Switching Language Modeling using Syntax-Aware Multi-Task Learning. Genta Indra Winata, Andrea Madotto, Chien-Sheng Wu, and Pascale Fung. In Proceedings of the Third Workshop on Computational Approaches to Linguistic Code-Switching\@ACL 2018, Melbourne, Australia, July 19, 2018.
\item End-to-End Dynamic Query Memory Network for Entity-Value Independent Task-Oriented Dialog. Chien-Sheng Wu, Andrea Madotto, Genta Indra Winata, and Pascale Fung. In 2018 IEEE International Conference on Acoustics, Speech and Signal Processing, ICASSP 2018, Calgary, AB, Canada, April 15-20, 2018.
\item Emo2Vec: Learning Generalized Emotion Representation by Multi-task Training. Peng Xu, Andrea Madotto, Chien-Sheng Wu, Ji Ho Park, and Pascale Fung. In Proceedings of the 9th Workshop on Computational Approaches to Subjectivity, Sentiment and Social Media Analysis, WASSA\@EMNLP 2018, Brussels, Belgium, October 31, 2018.

\end{itemize}
